Zero-shot Object Counting

Class-agnostic object counting aims to count object instances of an arbitrary class at test time. It is challenging but also enables many potential applications. Current methods require human-annotated exemplars as inputs which are often unavailable for novel categories, especially for autonomous systems. Thus, we propose zero-shot object counting (ZSC), a new setting where only the class name is available during test time. Such a counting system does not require human annotators in the loop and can operate automatically. Starting from a class name, we propose a method that can accurately identify the optimal patches which can then be used as counting exemplars. Specifically, we first construct a class prototype to select the patches that are likely to contain the objects of interest, namely class-relevant patches. Furthermore, we introduce a model that can quantitatively measure how suitable an arbitrary patch is as a counting exemplar. By applying this model to all the candidate patches, we can select the most suitable patches as exemplars for counting. Experimental results on a recent class-agnostic counting dataset, FSC-147, validate the effectiveness of our method. Code is available at https://github.com/cvlab-stonybrook/zero-shot-counting

==> backup.tex <==

An effective approach for class-agnostic counting is to count via a few visual exemplars of the object category. Based on these exemplars, we can obtain a correlation map between the exemplars and the input image, which indicates the densities of the object category across the whole image. In our setting where we do not have any human inputs during test time, the obvious question here is how to obtain the exemplars of an arbitrary class where the only input given is the class name.

\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.30\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
    Number of  & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    proposals & MAE & RMSE & MAE & RMSE \\
    \midrule
    150 & {27.21} & \textbf{87.77} & {22.54} & {120.88}  \\ 
    300 & {27.31} & {88.50} &  {23.01} & {124.02}  \\
    450 & \textbf{26.93} & {88.63} &  \textbf{22.09} & \textbf{115.17}  \\
    600 & {27.06} & {89.31} &  {22.63} & {115.26}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{ Performance when using different numbers of proposals. 
  } \vspace{-15pt} \label{tab:num_proposals}
\end{table}


\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.30\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
    $k$ & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    neighbors & MAE & RMSE & MAE & RMSE \\
    \midrule
    5 & {27.21} & \textbf{87.77} & {22.54} & {120.88}  \\ 
    10 & {27.31} & {88.50} &  {23.01} & {124.02}  \\
    25 & \textbf{26.93} & {88.63} &  \textbf{22.09} & \textbf{115.17}  \\
    50 & {26.99} & {88.59} &  {22.42} & {115.32}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{ Performance when selecting different numbers of class-relevant patches. 
  } \vspace{-15pt} \label{tab:num_K_near}
\end{table}

\begin{table}[!h] 
\vspace{-15pt}
  \centering
\resizebox{0.31\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
    Number of  & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    exemplars & MAE & RMSE & MAE & RMSE \\
    \midrule
    1 & {27.54} & {89.45} & \textbf{21.76} & {115.31}  \\ 
    2 & {27.10} & \textbf{88.44} &  {22.00} & \textbf{114.93}  \\
    3 & \textbf{26.93} & {88.63} &  {22.09} & {115.17}  \\
    4 & {26.99} & {88.59} &  {22.42} & {115.32}  \\
    %5 & {26.97} & {88.58} &  {22.79} & {116.01}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{ Performance when using different numbers of exemplars. 
  } \vspace{-15pt} \label{tab:num_k}
\end{table}

\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.28\textwidth}{!}{%
  \begin{tabular}{c|cccc}
    \toprule
    \# Proposals & 150 & 300 & 450 & 600 \\
    \midrule
    MAE & {27.21} & {27.31} & \textbf{26.93} & {27.06}  \\ 
    MSE & \textbf{87.77} & {88.50} &  {88.63} & {89.31}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{ Performance under different numbers of proposals. 
  } \vspace{-15pt} \label{tab:num_proposals}
\end{table}



\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.28\textwidth}{!}{%
  \begin{tabular}{c|cccc}
    \toprule
    %$k$ & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    $k$ neighbors & 5 & 10 & 25 & 50 \\
    \midrule
    MAE & {27.05} & \textbf{26.93} & {27.22} & {27.47}  \\ 
    MSE & {88.68} & {88.63} &  \textbf{88.28} & {88.54}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{ Performance under different $k$. 
  } \vspace{-15pt} \label{tab:num_K_near}
\end{table}

\begin{table}[!h] 
\vspace{-8pt}
  \centering
\resizebox{0.30\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
    Proposals  & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    for selection & MAE & RMSE & MAE & RMSE \\
    \midrule
    SS & {27.66} & {91.71} & {22.36} & {122.35}  \\ 
    ZSI & \textbf{25.98} & \textbf{86.74} & {22.28} & {117.77}  \\
    RPN & {26.76} & {87.41} & 23.52 & 126.68  \\
    Random & {26.93} & {88.63} &  \textbf{22.09} & \textbf{115.17}   \\
    %5 & {26.97} & {88.58} &  {22.79} & {116.01}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{Performance when using different types of proposals. 
  } \vspace{-15pt} \label{tab:candi_patches}
\end{table}

\begin{table}[!h] 
\vspace{-8pt}
  \centering
\resizebox{0.33\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
    Proposals  & \multicolumn{2}{c|}{Val MAE} & \multicolumn{2}{c}{Test MAE} \\
    for selection & w/o P.S. & w/ P.S. & w/o P.S. & w/ P.S. \\
    \midrule
    SS & {33.77} & {27.66} & {29.16} & {22.36}  \\ 
    ZSI & {32.10} & \textbf{25.98} & {26.96} & {22.28}  \\
    RPN & {32.19} & {26.76} & 29.25 & 23.52  \\
    Random & {35.14} & {26.93} &  {32.63} & \textbf{22.09}   \\
    %5 & {26.97} & {88.58} &  {22.79} & {116.01}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-8pt}
  \caption{Performance when using different types of proposals. 
  } \vspace{-15pt} \label{tab:candi_patches}
\end{table}

\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.35\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
      & \multicolumn{2}{c|}{$\geq$1 instances} & \multicolumn{2}{c}{$\geq$5 instances} \\
    & MAE & RMSE & MAE & RMSE \\
    \midrule
    %CFOCNet (1-shot) & {2.16} & {3.27} & {3.19} & {4.40}  \\ 
    CFOCNet (5-shot) & \textbf{1.90} & \textbf{2.80} &  {2.82} & {3.77}  \\
    Ours (0-shot) & {2.51} & {3.15} &  \textbf{2.53} & \textbf{3.17}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{-10pt}
  \caption{ Performance on COCO subset. 
  } \vspace{-15pt} \label{tab:coco}
\end{table}
